Certification of entangled quantum states and quantum measurements in Hilbert spaces of arbitrary dimension

The emergence of quantum theory at the beginning of 20$-th$ century has changed our view of the microscopic world and has led to applications such as quantum teleportation, quantum random number generation and quantum computation to name a few, that could never have been realised using classical systems. One such application that has attracted considerable attention lately is device-independent (DI) certification of composite quantum systems. The basic idea behind it is to treat a given device as a black box that given some input generates an output, and then to verify whether it works as expected by only studying the statistics generated by this device. The novelty of these certification schemes lies in the fact that one can almost completely characterise the device (up to certain equivalences) under minimal physically well-motivated assumptions such as that the device is described using quantum theory. The resource required in most of these certification schemes is quantum non-locality. In this thesis, we construct schemes to device-independently certify quantum states and quantum measurements in Hilbert spaces of arbitrary dimension along with the optimal amount randomness that one can extract from any quantum system of arbitrary dimension.

==> Template/random.tex <==
Throughout my PhD studies, many people helped me to finish my studies and finalize this thesis.
First of all, I would like to express my deep gratitude to my supervisor, Karol \.Zyczkowski.
Due to his constant mentorship, through my stipend at CFT and then PhD studies, I feel that I have gained a lot of insight into the world of science.
I can safely say that it would be extremely hard to finish the studies without his advice, both from the scientific and administrative perspectives.
At all times he was understanding and willing to help.  

Furthermore, I feel indebted to all the administrative team at CFT that helped me with numerous struggles to understand the policies needed to survive in the scientific community.
The other PhD students in room 304A made it a place that is worth coming -- the meeting of the quantum world and ``astrology'' provided a great environment.
Therefore, I would like to acknowledge the support of astrophysicists and cosmologists: Ishika Palit, Julius Sorbenta, Michele Grasso, and Suhani Gupta.

The thesis increased its quality due to numerous people that devoted their time to provide me with insights regarding corrections: Albert Rico, Arul Lakshimanarayan, Jerzy Paczos, my cousin Jim Borneman, Kamil Korzekwa, my sister Katarzyna, Marcin Wierzbi{\'n}ski, Tomasz Linowski, Vinayak Jagadish, and Wojciech Bruzda.
I express my gratitude to Konrad Szyma{\'n}ski for creating a 3D printout of the circulant set.

Having finished exactly 20 years of studies since the beginning of primary school, I feel grateful to my parents who always believed in me and provided every help they could.
It would be hard to express in words what their aid signifies to me. 

Finally, the person who has been my strongest supporter is my wife Paulina.
Her understanding and constant motivation meant everything to me during the research.
There are so many aspects in which she helped me that it would be impossible to mention them all.
Let me just mention the most visible support seen in this thesis, namely her artistic photographs that visualize scientific concepts.

% my wife

% all my collaborators

% 


%Vinayak Jagadish
